GTOC X: Solution Approach of Team Sapienza-PoliTo

This paper summarizes the solution approach and the numerical methods developed by the joint team Sapienza University of Rome and Politecnico di Torino (Team Sapienza-PoliTo) in the context of the 10th Global Trajectory Optimization Competition. The proposed method is based on a preliminary partition of the galaxy into several small zones of interest, where partial settlement trees are developed, in order to match a (theoretical) optimal star distribution. A multi-settler stochastic Beam Best-First Search, that exploits a guided multi-star multi-vessel transition logic, is proposed for solving a coverage problem, where the number of stars to capture and their distribution within a zone is assigned. The star-to-star transfers were then optimized through an indirect procedure. A number of refinements, involving settle time re-optimization, explosion, and pruning, were also investigated. The submitted 1013-star solution, as well as an enhanced 1200-point rework, are presented.

==> M11.tex <==
  \begin{tabular}{ccccc}
    &  8 &  9 &  10 &  11 \\ \cline{2-5} 
    \multicolumn{1}{c|}{23} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{2} \\ \cline{2-5} 
    \multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
    \multicolumn{1}{c|}{21} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
    \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
    \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} \\ \cline{2-5} 
    \multicolumn{1}{c|}{18} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
    \multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{9} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
    \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 1}} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
\end{tabular}

==> OLD.tex <==

\section{Abstract Esteso}


%\vspace{3mm}
This paper provides an overview of the solution approach and the numerical methods developed by the joint team Sapienza University of Rome and Politecnico di Torino (Team Sapienza-PoliTo) in the context of the \nth{10} Global Trajectory Optimization Competition, also known as GTOC X.

The proposed problem, named ``Settlers of the Galaxy'', 
represents a unique challenge, 
where participants are asked to design
a settlement tree for colonizing the galaxy, i.e., a pool of one hundred thousand candidate stars,
scoring points according to a prescribed merit function $J$, that rewards 
large settlements, uniformly distributed in space. An efficient use of propulsion is also taken into account as a multiplicative premium factor.
Solutions submitted earlier in the competition are also slightly rewarded.

A set of rules is provided, which constrains the number of starting vessels, namely Mother Ships and Fast Ships, as well as the number of new vessels, namely Settler Ships, that may depart from any settled star.
Maneuverability limits for each type of vessel, i.e., maximum number and magnitude of allowed velocity increments, are also assigned.
A peculiar, non-keplerian, central-force gravitational model 
is assumed for the motion of both stars and ships, 
inspired by the circular motion observed for actual stars in the Milky Way.

%\hl{volendo si possono aggiungere altre problem features - esplosione?}
The solution approach of Team Sapienza-PoliTo mostly depended on the identified problem features.
According to the analysis of the merit function $J$, 
the minimization of the error functions $E_r$ and $E_\theta$ was deemed essential for maximizing the score, hence it was assumed as main design goal.
Indeed, one should notice that if the error functions $E_r$ and $E_\theta$ are small, $J$ increases almost linearly with the number of settled stars $N$.

 A problem reformulation was devised in order not to deal directly with the error functions whilst providing an almost equivalent, yet more practical, way to handle the problem.
The galaxy  was partitioned according to a $30\times 32$ grid, defined over the ($r$, $\theta_f$) plane, where the $k_r$-th horizontal row (or ``ring'') was defined by $r\in \left[1 + k_r,\, 2 + k_r \right]$,  with $k_r \in [1,\,30]$, and the $k_\theta$-th column (or ``stripe") by  $\theta_f \in \left[-\pi + \frac{\pi}{16} (k_\theta-1),\, -\pi + \frac{\pi}{16} k_\theta \right]$, with $k_\theta \in [1,\,32]$.

Next, an optimal distribution of stars in each row and column for minimizing the error functions $E_r$ and $E_\theta$  was searched for,
by assuming the center of each grid cell as a proxy for the actual location of each star inside that cell.
This assumption was motivated by the fact that if the star distribution is sufficiently dense and the number of captured stars is sufficiently large, 
then the local effects would be minimal.

As a result of this analysis, it was found out that the errors could be kept to a minimum by a settlement tree of $512 \times n$ stars, equally-distributed over the 32 columns and linearly-distributed over the 30 rows, with more settled stars at the higher radii than at lower ones.
Given the limited team experience in dealing with very large data structures, as well as the short available time,  a decision was made to limit the number of settled stars to about 1020, postponing all the possible solution refinements to the last few days of the competition.
%
Randomly sampling stars according to the proposed distribution provided a (reasonable-enough) empirical proof for justifying the proposed problem reformulation.
Numerical investigations also suggested that small deviations from the target distribution leading to errors smaller than unity could be accepted without severely hindering the overall score.
Conversely, an unsupervised increment of the number of stars would have resulted in a significant score drop.


Given the small number of vessels at Year Zero,
the role of Settler Ship multiplication in creating the settlement tree was apparent.
Mobility charts were drawn for the Settler Ships in order to provide a graphical tool for assessing the maneuvering capability of a vessel, that is, the location of all reachable arrival stars in the ($r$, $\theta_f$) plane as a function of departure radius, flight time, and departure epoch.

A spiral occupation was recognized as the only viable option, being a global uniform coverage of the space unfeasible due to the strict time constraints. 
%
Settler Ship mobility charts were used for guiding the search of the opening maneuvers, that is,  Mother Ships  and Fast Ships trajectories departing from Sol at Year Zero.
In order to keep the search for the opening trajectories  simple enough, 
Mother Ship trajectories intercepting more than three stars had not been investigated.
The target number (1020) of settled stars  was so low that 
two or three ``root'' settlements per Mother Ship were deemed sufficient for attaining the desired number of settled stars. 
Opening maneuvers had been concurrently optimized in order to provide ``root'' settlements in galaxy locations sufficiently far apart  to allow 
a proper ``growth'' of the spiral settlement tree,
without having multiple ``sub-trees'' originating from different roots competing each other for the same stars.

Eventually, 9 non-overlapping zones, that is, sets of contiguous cells of the ($r$, $\theta_f$) grid, had been identified.
In each zone a set-covering problem is posed
as
finding the optimal settlement tree, for an assigned
departure (or ``root'') star and epoch,
that allows to settle a prescribed number of stars per cell within the zone.
An alternative formulation where the number of stars in each row and column (of a prescribed zone) is assigned, instead of cell-by-cell basis, was also investigated. 

A multi-settler stochastic Beam Best-First Search (BBFS) has been developed for solving this unusual problem, 
as a variant of the (single-spacecraft) ``Stochastic Beam'' algorithm proposed by Sim{\~o}es et al. \cite{simoes2017multi} for  handling the multi-rendezvous problem released in GTOC 5.
%
%Let us consider a \textit{search tree}, where each node, hereafter \textit{state}, represents a settlement tree, i.e., an un-ordered list of settled stars, each one labeled with information about i) the ``parent'' star (i.e., where the in-bound Settler Ship comes from), ii) the ``offspring'' stars reached by the out-bounding Settler Ships, and iii) the star settlement epoch.
%A visual representation of a settlement tree in the ($r$, $\theta_f$) plane is proposed in Figure~\ref{fig:tree}, where time information is neglected for the sake of clarity.
%A cost function $g = \|H - G\|$, that measures the difference between the actual number of settled stars $H(k_r,\,k_\theta)$ and the target one $G(k_r,\,k_\theta)$ in cell ($k_r,\,k_\theta$), is used for ranking the states in the search tree.
% 
%At the beginning, the search tree contains just one state, that is, the settlement tree made up only by the starting star, settled at a known epoch $t_{root}$.
%New states, or \textit{successors}, are built upon previously evaluated ones by using an incremental mechanism.
%
In the proposed beam-search variant, termed \textit{best-first}, only the best state is used for generating the successors states at any iteration. 
 
For each settled star
belonging to the selected, \textit{ancestor}, state, 
and with at least one available vessel, 
all reachable stars  within time and $\Delta V$ constraints are gathered, forming a \textit{reachable minimum-time} neighborhood.
In order to keep the computational time reasonably low,
only two-impulse trajectories are considered. Also, a linear dynamical model, based on the Hill-Clohessy-Wiltshire equations, is used for estimating the $\Delta V$ for moving from one star to another, for  assigned departure and arrival epochs, without solving the full optimization problem.
Only minimum-time transfers are considered, as this allows for easily creating large trees.
In order to speed-up the tree-search procedure, all reachable minimum-time neighborhoods in a zone are computed offline,
with departure and arrival epochs discretized over a uniform time-grid with a 1 Myr step size.

Among all possible successors, only a limited number  $b_{f,max}$ is retained and inserted in the search-tree.
This selection follows a set of stochastic rules that aim at rewarding successors states on the basis of both
their \emph{exploring} power (i.e., number of non-empty cells) and their \emph{exploitation} power (i.e., number of settled stars).

Subsequently, the search-tree frontier, that collects all unexplored states of the search-tree,
now containing a (possibly large) number of states evaluated at different iterations, is sorted according to the cost function $g$ and the best $b_w$ are kept in memory,
while the others are discarded.
The now-exhausted ancestor state is removed from the search-tree frontier, and a new iteration may begin.
The algorithm terminates as soon as successors can no longer be generated from any of the states in the frontier.
The best-so-far state is eventually elected as putative optimum for the zone set-covering problem.  


The best-first (or uniform-cost \cite{russell2016artificial}) variant has been here adopted in order to provide good-quality answers to each set-covering problem as soon as possible. 
Settlement trees of up to 100 stars were generated in a few minutes on a standard laptop.


The proposed procedure has been repeated over all zones,
iteratively changing the target occupancy distribution according to the attained results,
in order to have an overall number of settled stars in each row and column as close as possible to the one stated by the global target distribution devised beforehand.
Eventually, a settlement tree with $1013$ stars was found at the end of this first phase.



Each star-to-star transfer leg was recomputed by accounting for the complete problem dynamics. The two-impulse rendezvous trajectory was searched first. 
Then, in accordance with the problem constraints, up to two intermediate maneuvers were added to the two-impulse solution. Eventually, the settlement epochs of all states were globally adjusted leading to a small, yet significant, increase in the final value of the merit function. A visual representation of this solution is provided in Figure~\ref{fig:sol}. 

A quick analysis of the attained solution revealed that 
the actual distribution of captured stars was not as uniform as expected, and the total error $E_r + E_\theta$ larger than unity.
In addition, a significant number of settler ships capable of reaching at least one new star within the mission time-window  was still available. 
Therefore, the team last efforts in the competition were oriented towards finding a refined solution, with the aim of both increasing the total number of settled stars $N$, and possibly reducing, even slightly, the error functions.
In this fashion, an Integer Linear Programming (ILP) problem was defined,
whose solution provided the number of additional stars to settle in each cell, given the available number of vessels and their location in the ($r$, $\theta_f$) plane.
Unfortunately, the competition ended before we were able to process this refined solution. 



 
 


 


\section{Opening Maneuvers} \label{sez:MSFS}

\dots
\newline





Eventually, 9 non-overlapping zones, that is, sets of contiguous cells of the ($r$, $\theta_f$) grid, have been identified.
Each zone $\mathcal{Z}$ encompasses a number of rows $K_r^{\mathcal{Z}} = \{ k_r\, |\, k_{r,min} \leq k_r \leq k_{r,max}\}$ and columns $K_\theta^{\mathcal{Z}} = \{ k_\theta\, |\, k_{\theta,min} \leq k_\theta \leq k_{\theta,max}\}$, and it is labeled by two or three alpha-numeric characters: a letter, which indicates if the star is encountered by a Mother Ship ($M$) or a Fast Ship ($F$), respectively; a first number, which uniquely identifies the ship, and, for the Mother Ships, a second number that corresponds to the settled star number (ordered by settling time).
The identified zones are listed in Table~\ref{tab:zones}.

\begin{table}[h!]
    \centering
    \begin{tabular}{c | c c}
        $\mathcal{Z}$ & $K_\theta$ & $K_r$\\
         \hline
          $M11$ &  $8,11$ & $16,23$\\
          $M12$ &  $11,13$ & $20,25$\\
          $M21$ &  $2,5$ & $15,21$\\
          $M22$ &  $5,8$ & $20,25$\\
          $M31$ &  $21,28$ & $1,13$\\
          $M32$ &  $27,30$ & $6,13$\\
          $M33$ &  $31,2$ & $12,16$\\
          $F1$ &  $14,17$ & $26,30$\\
          $F2$ &  $18,21$ & $26,30$\\
          \hline
    \end{tabular}
    \caption{Identified zones. }
    \label{tab:zones}
\end{table}

\section{Searching for Settlement Trees} \label{sez:search}

In each of the 9 zones in Table~\ref{tab:zones}, a \textit{set-covering problem} is posed: for an assigned departure (or ``root'') star and epoch, the goal is to find the settlement tree that allows to settle, in the shortest possible time, a prescribed number of stars per cell within the zone.
So, a target \textit{distribution matrix} $G$ is defined in each zone $\mathcal{Z}$, where $G(k_r,\,k_\theta)$ indicates the number of stars to settle in cell ($k_r,\,k_\theta$), for each $k_r \in K_r^\mathcal{Z}$ and $k_\theta \in K_\theta^\mathcal{Z}$.
An example of such a distribution matrix is reported in Table~\ref{tab:M11} for the zone $M11$.

\begin{table}[h!]
\centering
%\begin{tabularx}{0.1\textwidth}{*{5}{X}}
\begin{tabular}{ccccc}
&  8 &  9 &  10 &  11 \\ \cline{2-5} 
\multicolumn{1}{c|}{23} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{2} \\ \cline{2-5} 
\multicolumn{1}{c|}{22} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
\multicolumn{1}{c|}{21} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
\multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{8} \\ \cline{2-5} 
\multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{6} \\ \cline{2-5} 
\multicolumn{1}{c|}{18} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
\multicolumn{1}{c|}{17} & \multicolumn{1}{c|}{9} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
\multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 1}} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} \\ \cline{2-5} 
\end{tabular}
\caption{Distribution matrix $G$ for zone $M11$. The red number indicates the root star.}
\label{tab:M11}
\end{table}

Initially, an alternative formulation where the number of stars was assigned in each row and column,
%of a prescribed zone, 
instead of cell-by-cell basis, had been also investigated.
Despite in this formulation the target distribution in a zone was simpler to devise starting from the reference $1020$-star solution previously described, the number or possible settlement trees complying with the assigned distribution is far greater with respect to the cell-by-cell case, so \hl{slowing/worsening} the search procedure. Moreover, by working with a cell-by-cell distribution, a same number of stars in a row (or column) can be achieved by leaving empty some of the cells along such row (or column), as clearly evident in Table~\ref{tab:M11}; as a result, all the stars in the empty cells can be discarded during the search procedure, which is thus further simplified. These reasons led us to prefer an objective distribution by cells instead of by rows and columns, in each of the identified zones.

\subsection{Search Problem} \label{sez:problem}
The set-covering problem stated at the beginning of this section can be re-formulated as a ``standard'' \textit{search problem} \cite{russell2016artificial}, where the objective is to look for a sequence of \textit{actions}, \emph{i.e.}, transitions from a state to the next one (or \textit{successor}), that, starting from a known initial state, reaches a \textit{goal} state, that is, an optimal state according to a given \textit{performance measure}.
%, more often a cost function to minimize.

In order to formally define the set-covering problem as a search problem, the following components must be specified: (i) the state space of the problem, that is, the set of all states reachable from the initial state by any sequence of actions, (ii) a performance measure, to compare the states each other and push the search towards the goal, and (iii) the transition model, which allows to generate the successors of a given state.

\subsubsection{State Space.} \label{sez:states}
Each state in the state space represents a settlement tree, i.e., an un-ordered list of stars $\mathcal{S} =\{ s_0, s_1, \dots, s_n\}$ settled at times $t_0 < t_1 \leq \dots \leq t_n$. The k-th star $s_k$ is labeled with information about: i) the star ID, $ID_k$, ii) the ``parent'' star, $s_p$, where the in-bound Settler Ship comes from, iii) a maximum of three ``offspring'' stars, $\mathcal{O}_k = \bigcup_{i = 1}^{l \leq 3} s_{o_i}$, reached by the out-bounding Settler Ships, and iv) the star settlement epoch $t_k$.
Since only the minimum (2-Myr) waiting time has been considered at each settled star, the evaluation of the transfer time from a parent star to any of its offspring is straightforward, once the settlement epochs are known.
The initial state of the search procedure is the settlement tree made up only by the starting star $s_0$, settled at a known epoch $t_0$.
A visual representation in the ($r$, $\theta_f$) plane of the best settlement tree obtained in zone $M11$ is proposed in Figure~\ref{fig:tree}, where time information is neglected for the sake of clarity.

\begin{figure} [h!]
    \centering
    \includegraphics[width=0.5\linewidth]{Figures/Tree.png}
    \caption{Settlement tree obtained in zone $M11$ as a result of the search procedure. The target distribution is reported in Table~\ref{tab:M11}.}
    \label{fig:tree}
\end{figure}

\subsubsection{Performance Measure.} \label{sez:cost}
The explored states are ranked according to the following cost function (to be minimized):
\begin{equation}
    g = \|H - G\| + \frac{t_n}{100}
    \label{eq:g}
\end{equation}
where, for each cell ($k_r,\,k_\theta$) composing the considered zone, $H(k_r,\,k_\theta)$ is the actual number of stars settled in that cell, and $t_n$ is the final settling time in Myr.
Being $\|H - G\|$ an integer value and $\frac{t_n}{100} < 1$, the final settling time becomes important only once the target distribution has been achieved.

\subsubsection{Transition Model.} \label{sez:successors}
New states, or \textit{successors}, are built upon previously evaluated ones by using an incremental mechanism.
For each ``fertile'' settled star $s_k$, \emph{i.e.}, with at least one available vessel ($|\mathcal{O}_k| < 3$), belonging to the selected, \textit{ancestor}, state $\mathcal{S}$, all reachable stars in the considered zone within time and $\Delta V$ constraints are gathered, forming a \textit{reachable minimum-time} neighborhood:

\begin{equation}
    \mathcal{N}_k = \{ s_h\, |\, t_h < 90\,\mbox{Myr} \wedge \Delta V(k,h,t_k + 2,t_h) < 350\,\mbox{km/s} \}
    \label{eq:Nk}
\end{equation}
where $\Delta V(i,j,t_i,t_j)$ is the velocity variation needed to move from star $s_i$ to star $s_j$, departing at epoch $t_i$ and arriving at epoch $t_j$.

%In order to keep the computational time reasonably low, only two-impulse trajectories are considered. Moreover, a linear dynamical model, based on the Hill-Clohessy-Wiltshire equations \cite{wh1960terminal}, is used for estimating the $\Delta V$ for moving from one star to another, for assigned departure and arrival epochs, without solving the full optimization problem.
In order to keep the computational time reasonably low, the linear dynamical model based on the Hill-Clohessy-Wiltshire equations \cite{wh1960terminal}, introduced in Section~X, is used for estimating the $\Delta V$ along a two-impulse trajectory connecting one star to another, for assigned departure and arrival epochs, instead of solving the full optimization problem.
Only minimum-time transfers are considered towards any reachable star, as this allows for easily creating large trees.
In order to speed-up the search procedure, all reachable minimum-time neighborhoods in a zone are computed offline,
with departure and arrival epochs discretized over a uniform time-grid with a 1 Myr step size.
Moreover, so as to reduce the state space dimension, at each point of the search process the non-settled stars located in already filled cells (in accordance with the distribution matrix $G$) are removed from the neighborhoods.

Given the adopted encoding, a successor of state $\mathcal{S}$ is any state $\mathcal{S}' = \mathcal{S} \cup \mathcal{S}_A$ , with $\mathcal{S}_A$ an adjunct to $\mathcal{S}$ defined as:
\begin{equation}
\mathcal{S}_A = \left \{ s_m\, |\, \exists k \in [0,n] : |\mathcal{O}_k| < 3 \wedge s_m \in \mathcal{N}_k \setminus \mathcal{S} \right \}
\label{eq:successor}
\end{equation}

Simple mathematics allowed us to perform a rough evaluation of the maximum number of successors of any state during the search: by supposing that $n_f$ is the number of ``fertile'' stars, each with no offspring and a number of non-settled neighbors equal to $n_N$, the correspondent number of successor states is: 
\begin{equation}
    n_{succ} = \sum_{i=1}^{n_f} \binom{n_f}{i}  \sum_{j=1}^{3} \binom{n_N}{j}
\end{equation}
If common values are used for $n_f$ and $n_N$, a value greater than $10^{10}$ is easily obtained for $n_{succ}$.
For this reason, memory and time requirements forced us to limit to a maximum value $b_{f,max}$ (the greatest possible) the number of successors which can be generated by each state.

It became therefore necessary to devise a constructive heuristics for the successors' generation, that would have allowed us to focus the search towards the most promising regions of the state space, so as to mitigate, as much as possible, the intrinsic incompleteness of the search procedure.
The devised heuristics follows a set of stochastic rules that aim at generating successors states on the basis of both
their \emph{exploring} power (i.e., number of non-empty cells) and their \emph{exploitation} power (i.e., number of settled stars).

The successors are generated by means of an iterative procedure. Initially, the list of successor states is composed by the ancestor state only: $List = \{ \mathcal{S} \}$. At the end of any iteration of the \textit{generation procedure}, $n_{succ}$ new successors states are generated and inserted in $List$, replacing the existing ones.
The transition model, which allows to fill the container $List$, consists of four steps:
\hl{k e' usato sia come indice di stella che come indice di ciclo ecco perche' non capivo nulla}

\begin{enumerate}
    \item First, the fertile stars in the ancestor state $\mathcal{S}$ are ranked by using as ``fitness'' the number of missing stars (\emph{i.e.}, still to settle) in their own cell $(k_r, k_\theta)$ and in the 8 adjacent cells:
    %by looking at $G$.
    \begin{equation}
        f = \sum_{i=-1}^{1} \sum_{j=-1}^{1} \left [ G(k_r + i, k_\theta + j) - H(k_r + i, k_\theta + j) \right ]
    \end{equation}
    Then, a fertile star $s_k$ is selected among the candidates (and removed from the list) by means of a biased sampling without replacement, proportional to $f$. In such a way, it is promoted the creation of branches directed towards the most empty cells of the zone.
    \item Now, $m*|L^k|$ new successors states are created,
    by appending $m$ differently generated  set offspring of star $s_k$ to  to each state in $L^k$,
 
%    \item Now, $n_{succ} \times n_{succ}^k$ new successors states are going to be created by appending to each of the $n_{succ}$, already generated, (partial) successor states in $List$ a different group of offspring of star $s_k$.
    
      
    In order to reward stars with a fitness larger than the average these stars are allowed to generate 20\% more successors, to further encourage exploration, that is: 
    \begin{equation}
    \begin{array}{cc}
         m_k &=
         \begin{cases}
         1.2\, \hat m & \mbox{if}\,\,\, f_k > \bar{f} \\
         n_{succ}^{u} & \mbox{otherwise}
         \end{cases}
    \end{array}
    \label{eq:nsucck}  
    \end{equation}
    where 
    \hl{ $n_{succ}^{u} = \hat m \in [1,9]$ is tuning parameter that may be constant or randomly sampled at any iteration} - 
    %$n_{succ}^{u} = \left \lfloor b_{f,max}^{\frac{1}{n_{f}}} \right \rfloor$ is the number of successors that each of the $n_{f}$ fertile stars should generate so that to reach a total of $b_{f,max}$, 
    and $\bar{f}$ is the average fitness of the fertile stars.
    \item The number of offspring $n_{o}^k$ of the star $s_k$, to insert in each of the $n_{succ} \times n_{succ}^k$ new successors, is sampled in the range $\left [1, 3 - | \mathcal{O}_k | \right]$ with a probability proportional to itself. 
    The aim is to rapidly increase the number of settled stars in the settlement tree.
    \item Finally, each offspring star $s_o$
    %, reached by the out-bounding Settler Ships,
    must be selected within the neighborhood $\mathcal{N}_k$ of the parent star $s_k$.
    Settler Ship mobility charts suggested that a good strategy to fill, the fastest as possible, all the cells composing a zone is to alternate great ``leaps'' from cell to cell, moving along rows, and quick ``reproduction'' phases, for expanding along columns; such a strategy was named \textit{throw and multiply}:
    \begin{equation}
    \begin{array}{cc}
         s_o &=
         \begin{cases}
         \argmin_{s_h \in \mathcal{N}_k} (t_h - t_k) & \mbox{if}\,\,\, p_r < 0.5 \\%[10pt]
         \argmax_{s_h \in \mathcal{N}_k} \frac{|\Delta \theta_f|}{t_h - t_k} & \mbox{otherwise}
         \end{cases}
    \end{array}
    \label{eq:succ_choice}  
    \end{equation}
    being $p_r$ a random number between 0 and 1 and $\Delta \theta_f$ the difference in final polar angle between star $s_h$ and $s_k$.
    At this point, $s_o$ is removed from $\mathcal{N}_k$ and another offspring star is selected with the same rule, until $n_{o}^k$ offspring are generated.
    The $n_{o}^k$ offspring are appended to one of the $n_{succ} \times n_{succ}^k$ successors, and the process is repeated for each of them.
\end{enumerate}
The steps from 1. to 4. are repeated until the number of generated successors is equal to $b_{f,max}$.

\subsection{Beam Best-First Search} \label{sez:BBFS}
A multi-settler stochastic Beam Best-First Search (BBFS) has been developed for solving the unusual search problem defined in the previous section,
%as a variant of 
as a generalization of the (single-spacecraft) ``Stochastic Beam'' algorithm proposed by Sim{\~o}es et al. \cite{simoes2017multi} for  handling the multi-rendezvous problem released in GTOC 5. 
Solution methodologies based on the beam search have been demonstrated to be successful also in other GTOCs, characterized by a wide search space \cite{grigoriev2013choosing, izzo2013search, izzo2016designing, petropoulos2017gtoc9}.

%A search algorithm gradually builds a so-called \textit{search tree} by analyzing all (of most of all) the action sequences starting at the initial state, which constitute the ``root', trying to approach the goal. 
Being the beam search a \textit{tree-search} algorithm, it tries to approach the goal gradually building a so-called \textit{search tree}, with the initial state as root: 
the \textit{nodes} of the tree correspond to the explored states in the state space of the problem, while the \textit{branches} correspond to state-to-state transitions.

At each iteration, the algorithm picks the first \textit{leaf} state in the \textit{frontier}, that is, the list of all the generated, but yet unexplored, nodes at any given point of the search, and \textit{expands} it by generating a set of \textit{successor} states. 
In the proposed beam search variant, termed \textit{best-first}, the frontier is modeled as a priority queue ordered by $g$. So, at any iteration, the best state is used for generating $b_{f,max}$ successors states. A probabilistic branching is now exploited so as to further reduce the computational burden: with a probability $p$, the best $b_f$ successor states, according to $g$, are retained and appended to the frontier; otherwise, the $b_f$ nodes are chosen by means of a biased sampling without replacement proportional to $g$.
Subsequently, the frontier, now containing a (possibly large) number of states evaluated at different iterations, is sorted according to the cost function $g$ and the best $b_w$ are kept in memory, while the others are discarded.
The now-exhausted ancestor state is removed from the search-tree frontier, and a new iteration may begin.
The algorithm terminates as soon as successors can no longer be generated from any of the states in the frontier, or a maximum, pre-defined, number of nodes have been explored. The best-so-far state is eventually elected as problem solution. 

The best-first (or uniform-cost \cite{russell2016artificial}) variant has been here adopted, in place of the ``standard'' breadth-first search, in order to provide good-quality answers to each set-covering problem as soon as possible: indeed, as shown in Figure~\ref{fig:tree_search}, the best-first variant is able to cross freely the different levels of the tree and quicker generate ``deeper'' nodes (\emph{i.e.}, states with a larger number of settled stars), that we expect have a better solution score. 
In this way, settlement trees of up to 100 stars were generated in a few minutes on a standard laptop.

\begin{figure} [h!]
\centering
\begin{subfigure}{0.7\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BS.pdf}
  \caption{Beam (breadth-first) Search.}
  \label{fig:BS}
\end{subfigure}
\begin{subfigure}{0.7\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/BBFS.pdf}
  \caption{Beam Best-First Search.}
  \label{fig:BBFS}
\end{subfigure}
\caption{Comparison between six iterations of a breadth-first and best-first version of the Beam Search on the same problem, by supposing $b_f = 2$ and $b_w = 3$. Grey-filled nodes have been explored, while white-filled nodes have been generated but not yet explored. Instead, black-dashed nodes are yet to be generated, while grey-dashed nodes have been pruned by the beam procedure. In particular, red-crossed nodes are excluded by the probabilistic branching ($b_f$), while blue-crossed nodes by the frontier re-sizing ($b_w$). The values of the cost function $g$ are labeled in decreasing order: $g_j < g_i$ if $j > i$.}
\label{fig:tree_search}
\end{figure}

\hl{altri commenti?}

The hyper-parameters of the BBFS procedure were tuned ``by hand'' during the competition, by trying different values and comparing the correspondent results. At the end, the following values resulted to be the best ones for the great part of the analyzed zones: $b_w = 20000$, $b_{f,max} = 10000$, $b_f = 1000$.
In order to mitigate potential issues due to the ``non-exhaustiveness'' and stochastic nature of the BBFS, several runs were performed in parallel, and the best-found solution saved.

The proposed procedure has been repeated over all zones,
iteratively changing the target occupancy distribution according to the attained results,
in order to have an overall number of settled stars in each row and column as close as possible to the one stated by the global target distribution devised beforehand.
Eventually, a settlement tree with $1013$ stars was found at the end of this first phase.


\section{Full Transfers Optimization}
%\input{optimization.tex}



==> adjust.tex <==
\newpage
\section{Adjust Sequence Program}
The solution attained by the beam search algorithm, has been adjusted in order to reduce the $E_r$ error of each ring by replacing one star $j$ by another one $j^*$ with a more convenient radius.

First of all, the algorithm decides which star should be discarded.
In order not to cut off entire branches of the computed settlement tree, only terminal stars, i.e., stars from which no settler is scheduled to depart, are taken as candidates.
Among the candidate stars, if the mean radius of the settled stars in a ring is above the mid radius of the ring then the star on the lowest orbit is removed, otherwise the star with the greatest radius is picked for elimination.

Second, the optimal radius of the new star $r_{j^*}$ has to be computed.
Let us consider the error in each ring:
\begin{equation}
	E_r^{(k)} = \left( \frac{f_r(R_k)}{g_r(R_k)} - 1 \right)^2
\end{equation} 
for $k = 0, \dots , 29$. 
Notice that the error $E_r^{(30)}$ is not taken into account in this optimization.
Indeed, since a greater sensitivity of the error functions has been detected in the lower rings, we decided to minimize the $E_r$ relative to the lower bound of each ring.  
Hence, the error $E_r^{(30)}$, that is relative to the upper bound of the highest ring is cut off from the procedure.
Ideally we want the error to be null for each $k$, so we have to impose:
\begin{equation}
	f_r(R_k) = g_r(R_k)
	\label{eq:f_r_equal_to_g_r}
\end{equation} 
If $N$ denotes the total number of settled stars in all rings, $f_r(R_k)$ has the following expression:
\begin{equation}
	f_r(R_k) = \frac{1}{N} \left[ \sum\limits_{\substack{i = 1 \\ i \neq j}}^{N} f(R_k ; r_i, s_r) + f(R_k ; r_{j^*} , s_r) \right]
	\label{eq:f_r_k_with_sum}
\end{equation}
where $s_r = 1$ kpc and:
\begin{equation}
	f(x; \mu, s) = \begin{cases}
	0 & |x - \mu| \geq s \\
	\frac{1}{s} - \frac{|x - \mu|}{s^2} & \text{otherwise}
	\end{cases}
\end{equation}
Since the stars, other than $j$, are retained, the sum in Eq.~\eqref{eq:f_r_k_with_sum} is a constant, denoted by $\tilde{S}$.
By substituting $f_r(R_k)$ from Eq.~\eqref{eq:f_r_k_with_sum} in Eq.~\eqref{eq:f_r_equal_to_g_r} one obtains:
\begin{equation}
	r_{j^*} = R_k + (1 - s_r (N g_r(R_k) - \tilde{S})) s_r
	\label{eq:optimal_radius_adjust}
\end{equation}
where we assumed $r_{j^*} \in \left[R_k, R_k + s_r \right]$.
Equation~\eqref{eq:optimal_radius_adjust} provides the optimal radius.
At this point, the actual new star to be settled is looked for among the list of reachable stars.
The one with the radius closest to the optimal one is picked.

==> optimization.tex <==
The ships' trajectories are evaluated according to the dynamical model assumed for the competition. The position and velocity vectors are defines as $\bfr$ and $\bfV$, respectively, with
\begin{equation}
\dot \bfr = \bfV \hspace{2cm} \dot \bfv = \bfg(\bfr)
\end{equation}
where $\bfg$ is the gravitational acceleration vector.

The basic maneuver is a two-impulse transfer between two stars with fixed departure and arrival time. The solution is equivalent to Lambert's problem in Keplerian dynamics: the initial velocity components (three unknowns) must be determined in order to match the target position at the arrival time (three boundary conditions). The problem has a single solution and is not subject to optimization. It is worth noting that the trajectories improve when the time of flight is increased, as the competition overall time constraint forces time of flight that are much shorter than the optimal time (e.g., the equivalent of a Hohmann transfer).

Two-impulse maneuvers are usually optimal but impulses may be larger than allowable limits, either on single impulse magnitude and/or on overall $\Delta V$ value. Trajectories exceeding limits must be discarded for fastships, which can perform at most two impulses.
Instead, more impulses are available for motherships and settlerships, and multiple impulse trajectories are sought when necessary.

A multiple impulse trajectory can be subject to optimization and an indirect approach\cite{bryson,impulse,lowt} is used for this purpose.
The Hamiltonian is defined $H= \bflambda_r \bfV + \bflambda_V \bfg$ and the Euler-Lagrange equations are derived for the adjoint variables:
\begin{equation}
\dot \bflambda_r^T = -\partial H/\partial \bfr  \hspace{2cm} \dot \bflambda_V^T = -\partial H/\partial \bfV
\end{equation}
The problem is completed by the boundary conditions on state variables, that must ensure reaching the target and fulfilling the $\Delta V$ limitations, and boundary conditions for optimality.

For settlerships, up to 4 impulses are considered (no trajectory requiring 5 impulses has been found). The sum of impulse magnitudes is minimized; constraints on initial and/or final impulse magnitude are introduced when limits are exceeded. The boundary conditions for optimality require impulses parallel to the velocity adjoint vector (primer vector) and the same primer magnitude at non-constrained impulses. The primer magnitude must be maximum at intermediate impulses when the time is not constrained; however, this would lead to violation of the minimum time between maneuvers and the corresponding times must therefore be constrained.  

Motherships have encounters with multiple stars but are treated with a similar approach to minimize the overall $\Delta V$. Two classes of trajectories have been exploited in the solution: initial impulse-intercept-impulse-intercept-impulse-intercept and initial impulse-impulse-intercept-impulse-intercept. Again constraints on $\Delta V$s are introduced when limits are exceeded. Impulses are always at the minimum allowable time. Intercept times are left free and the conditions for optimality requires that the dot product of primer and pod $\Delta V$ is zero.




\cite{Casalino1998}
\cite{Casalino1999}
\cite{Bryson1979}





==> scarti.tex <==
\hl{------------------------------------------------------------}

Multi-impulses solution in a linear gravity field are generally more difficult to dealt with.

However, for the problem at hand, 
inner impulses, if needed, are located as close as possible to the starting/final ones,
being 

This is due to the fact that optimal solution is usually two impulse, and only the impulse

A relatively fast solution of a 
Four-impulse time-fixed linear rendezvous problem
can also be attained for this specific problem
by assuming that the magnitude constraints and impulse time separation constraints 
\hl{richeidono quella soluzione}.
%


The Four-impulse time-fixed linear rendezvous problem
with assigned inner maneuvering times can be posed as a convex problem,
and thus solved readily.


\hl{formulazione}

\hl{esempio di un caso}


\hl{------------------------------------------------------------}


\hl{commenti}

Validity of the proposed approach is verified by ...
\hl{confronto con la soluzione ottimale?}







Minimum time neighborhood
have been defined

In order to keep the computational cost as low as possible,


Analytical solution of the two-impulse time-fixed linear rendezvous problem is used 
to find time-minimum DV-constrained transfer from any departure start
to any other arrival star, as a function of the starting time.


A simple line search provide 



Time-minimum DV-constrained neighborhood
are defined as the set of all stars reachable from a given start at a starting time 








Linear multi-impulsive rendezvous problem has also been investigate
%
The problem solved is that of minimizing the total weighted characteristic velocity of a spacecraft subject to general linear equations of motion. 









 

the solution of the rendezvous problem of a vessel 
starting from a star $i$ at epoch $t_i$ and arriving at a star $j$ at time $t_j$
is provided by 

 





the equations of motion are linearized about a reference point or satellite
in a nominal orbit.

All of the aforementioned work that includes impulsive trajectories
based on linearized equations about a specific orbit (Refs. 1-10) utilizes a
nominal orbit that is circular, and most of these (Refs. 4-10) represent the
linearization through the Clohessy-Wiltshire equations. 




Section 2 includes a formulation of the general linear impulsive problem





In order to restric the possibilities
among all possible transfer,





DV impulse magnitude.
can be found iterating on the generic transfer time $\tau_f$.
In practice, a simple grid seach on a time discretization /time unit of 1 Myr was considered 









Analytical solution of the two-impulse time-fixed linear rendezvous problem is used 
for solving the 

two-impulse time-minimum DV-constrained linear rendezvous problem,
so that 





transfer from any departure start
to any other arrival star, as a function of the starting time.

time-Minimum DV-constrained two-impulse linear rendezvous 



This formulation is adopted in order to generate 
Minimum time neighborhood $\mathcal{N}(i,\,t_0)$
that is the set 
of all time-minimum transfer for a given sta











For the sake of clasirity,
a tree

This costructive heuristic is based on

tree of temporary/intermediate successor states is generated.

, as shown in Figure~\ref{fig:tree-heu}.
The ancestor state serves as root and is thus named "root state/root anchestor".




For the sake of clarity,

Let $\mathcal{T}$ be a


First, the fertile stars in the ancestor  $\mathcal{S}$ are ranked with respect to a function $f$ that measures the number of missing stars (\emph{i.e.}, yet to be settled) in the star cell $(k_r, k_\theta)$ and in the 8 adjacent cells:
    %by looking at $G$.
    \begin{equation}
        f = \sum_{i=-1}^{1} \sum_{j=-1}^{1} \left [ G(k_r + i, k_\theta + j) - H(k_r + i, k_\theta + j) \right ]
    \end{equation}

Biased Sampling without Replacement a biased sampling without replacement, with probability proportional to $f$, is used to sort fertile stars.
The $k$-th fertile star is going to be used as departure star for the creation of intermediate stages of tree depth $k$, regardless of intermediate (ancestor state).

The idea is to promote the creation of branches directed towards the most empty cells of the zone. 


%Level-1 intermediate successor are created by selecting 
Then,
a fertile star $s_k$ belonging to the ancestor is chosen and
a number of successors are generated by a 
\textit{single-star multiple-vessel} mechanism,
that is up to 3 vessels, according to the \hl{star availability},
are used to settle new stars belonging to the minimum time hill neighborhood $N_k$.

hl{qui descrivo in dettaglio cosa si fa}

scelgo una stella di partenza 
usando bias sampling stocastic sampling where the probability
of chosing a fertile star $s_k$ is proportional to its fitness

f

This pemette di ...

estraggo un numero da uno a 3
colonizzo in base alle regole 

ripeto m volte per creare 



















at the end of the first stage, $d_1$ level-1 intermediate states are created, forming the tree level 1.

In order to create level-2 intermediate states
another fertile star of the root state is chosen  and all 
level one intermediate states are now "exploded"
according to the same \textit{single-star multiple-vessel mechanism};

this procedure is repeated until one level contains at least $b_{f,max}$ states or it is not possible to generate new states (typically because all neighborhoods are empty ).

these $b_{f} \le b_{f,max}$ terminal states \hl{costituiscono l'output del meccanismo di generazione multi-stella multi-vessel}


\hl{********************************************************}






Several transition models may be defined for the problem under investigation.
The one adopted in the present work is a multi-star multi-vessel transition model,
that is 
in a single transition, up to three vessels may depart from any number of 
``fertile'' star in  ancestor state $\mathcal{S}$ for settling new stars,
that will be added to the successor state $S'$.


A huge number of successors can be generated 
by considering all possible combination of departure and arrival stars, 
letting aside the travel time, which is assumed to be the minumum transfer time according to the hill neighborhood.
For an ancestor state $S$ with $n_f$ ``fertile'' stars and an average neighborhood size $n_N$, 
up to $ n^{max}_{s'} = \sum_{i=1}^{n_f} \binom{n_f}{i}  \sum_{j=1}^{3} \binom{n_N}{j}$ successors can be approximately generated.




The number of successors  increases exponentially as the settlement tree grows is apparent; \hl{la situazione peggiora} as  the star density increases, that is for radii less then 5.

Memory constraints prohibit the generation of all possible successors;
only a limited number of successors $b_{f,max}$ will be generated.
A careful choice of the heuristic  rule governing the generation of the successors is thus of prime importance
\hl{in order to drive the creation (and consequently the search),
towards the most promising regions of the state space, mitigating, as much as possible, the intrinsic incompleteness of the search procedure.
}



The adopted procedure requires to define a number of intermediate successor states,
organized as a tree, as shown in Figure~\ref{fig:tree-heu} 


The ancestor state is designed as "root ancestor" and used as a root for the tree.

%Level-1 intermediate successor are created by selecting 

Then,
a fertile star $s_k$ belonging to the ancestor is chosen and
a number of successors are generated by a 
\textit{single-star multiple-vessel mechanism},
that is up to 3 vessles, according to the \hl{star avaiability},
are used to settle new stars belonging to the minimum time hill neighborhood $N_k$.

at the end of the first stage, $a_1$ intermediate states are created, forming the tree level 1.

level one intermediate states are now "exploded"
according to the 
\textit{single-star multiple-vessel mechanism}, but choosing (for all states at this level) a (not already used) fertile star of the root anchestor.

this procedure is repeated until one level contains at least $b_{f,max}$ states or it is not possible to generate new states (typically becouse of empty neighborhoods)

these $b_{f} \le b_{f,max}$ terminal states \hl{costituiscono l'output del meccanismo di generazione multi-stella multi-vessel}

















Given an ancestor state $\mathcal{S}$,
a huge number of successors can be generated 
by considering all possible combination of 
stars that could be settled using up to three vessel from any (already settled) ``fertile'' star in  $\mathcal{S}$.


A least-distance transition model, or one-vessel transition,
involves the creation of a number of successor states $\mathcal{S}'$ that differs from $S$ just by one element.

this transition model requires to select a "fertile" stars of S, $s_k$ and then settle one star in the hill minimum time hill neighborhood 




\hlc[green]{-------------------------------------------}



Given an ancestor state $\mathcal{S}$ a successor $\mathcal{S}'$


multiple-star multiple vessel transition

one-vessel transition/generation rule 



 


Given an ancestor state $\mathcal{S}$,
a huge number of successors can be generated 
by considering all possible combination of 
stars that could be settled using up to three vessel from any (already settled) ``fertile'' star in  $\mathcal{S}$.

Approximately, up to $ n^{max}_{s'} = \sum_{i=1}^{n_f} \binom{n_f}{i}  \sum_{j=1}^{3} \binom{n_N}{j}$ successors can be found 
For an ancestor state $S$ with $n_f$ ``fertile'' stars and an average neighborhood size $n_N$.
The exponential growth in the number of successor as the settlement tree grows is apparent.
The number increases with star density. \hl{cioe' nelle zone basse}


Due to memory constraints, only a limited number of successors $b_{f,max}$ can be generated.
An heuristic rule  is used in order to drive the creation (and consequently the search),
towards the most promising regions of the state space, mitigating, as much as possible, the intrinsic incompleteness of the search procedure.

A variety of stochastic rules has been devised for generating successors states on the basis of both
their \emph{exploring} power (i.e., number of non-empty cells) and their \emph{exploitation} power (i.e., number of settled stars).


The proposed procedure ``esplodes'' many (if not all) fertile stars  , in a given order, until $n^{L}_{succ}$ successors are generated.

The proposed procedure ``esplodes'' fertile stars, in a given order, 
until $n^{L}_{succ}$ successors are generated.








Each of intermediate successor (del livello L) is further ``exploded'' 
according to the same rule in order to create producendo $n^{L+1}_{succ}$ successori

This hybrid bredth-

stocastic 


breadth first search to generate




The number of offspring $n_{o}^k$ of the star $s_k$, to insert in each of the $n_{succ} \times n_{succ}^k$ new successors, is sampled in the range $\left [1, 3 - | \mathcal{O}_k | \right]$ with a probability proportional to itself. 
    The aim is to rapidly increase the number of settled stars in the settlement tree.
    
     Finally, each offspring star $s_o$
    %, reached by the out-bounding Settler Ships,
    must be selected within the neighborhood $\mathcal{N}_k$ of the parent star $s_k$.
    Settler Ship mobility charts suggested that a good strategy to fill, the fastest as possible, all the cells composing a zone is to alternate great ``leaps'' from cell to cell, moving along rows, and quick ``reproduction'' phases, for expanding along columns; such a strategy was named \textit{throw and multiply}:
    \begin{equation}
    \begin{array}{cc}
         s_o &=
         \begin{cases}
         \argmin_{s_h \in \mathcal{N}_k} (t_h - t_k) & \mbox{if}\,\,\, p_r < 0.5 \\%[10pt]
         \argmax_{s_h \in \mathcal{N}_k} \frac{|\Delta \theta_f|}{t_h - t_k} & \mbox{otherwise}
         \end{cases}
    \end{array}
    \label{eq:succ_choice}  
    \end{equation}
    being $p_r$ a random number between 0 and 1 and $\Delta \theta_f$ the difference in final polar angle between star $s_h$ and $s_k$.
    At this point, $s_o$ is removed from $\mathcal{N}_k$ and another offspring star is selected with the same rule, until $n_{o}^k$ offspring are generated.
    The $n_{o}^k$ offspring are appended to one of the $n_{succ} \times n_{succ}^k$ successors, and the process is repeated for each of them.












The successors generation procedure is here described.






\hlc[green]{LF - controlalre}
a temporary list of successor states is created.














 




is based on the repeated application of a partial-construction rule
that
given a (temporary) state $ \mathcal{S}$ creates $m$
(temporary) states $\mathcal{S}'$

where 


similarly to a breadth search

\hl{------------------------------------------------------------------------}













Given an ancestor state with $n_f$ ``fertile'' stars and an average neighborhood size $n_N$, a rough evaluation of the potential number of successors is given by

%\hl{il punto e' che non manda una nave ma ne manda tante per ogni transizione
%Questa operazione fa si che lo spazio di ricerca resti lo stesso, 
%ma le transizioni - freccie che connettono gli stati - sono molte molte di piu'. una riflessione su questo punto e' opportuna
%}

\begin{equation}
    n_{succ} = \sum_{i=1}^{n_f} \binom{n_f}{i}  \sum_{j=1}^{3} \binom{n_N}{j}
\end{equation}

Typical values of $n_f$ and $n_N$ for a settlement tree/state 
in between of the search process are \hlc[green]{LF-inserire}.
that is, up to $10^{10}$ could be created from one state.
The number increases with star density. \hl{cioe' nelle zone basse}


As a result, this formulation does not allow to explore (or even to generate) all possible successors of a state.
Therefore, only a limited number of successors $nxx$ is generated, 
according to some heuristic rules,
that 
strive to drive the search towards the most promising regions of the state space, mitigating, as much as possible, the intrinsic incompleteness of the search procedure.

A variety of stochastic rules has been devised for generating successors states on the basis of both
their \emph{exploring} power (i.e., number of non-empty cells) and their \emph{exploitation} power (i.e., number of settled stars).

The successors generation procedure is here described.

\hlc[green]{LF - controlalre}
a temporary list of successor states is created.


Initially, the list of successor states is composed by the ancestor state only: $List = \{ \mathcal{S} \}$. At the end of any iteration of the \textit{generation procedure}, $n_{succ}$ new successors states are generated and inserted in $List$, replacing the existing ones.
The transition model, which allows to fill the container $List$, consists of four steps:
\begin{enumerate}
    \item First, the fertile stars in the ancestor state $\mathcal{S}$ are ranked with respect to a function $f$ that measures the number of missing stars (\emph{i.e.}, yet to be settled) in the star cell $(k_r, k_\theta)$ and in the 8 adjacent cells:
    %by looking at $G$.
    \begin{equation}
        f = \sum_{i=-1}^{1} \sum_{j=-1}^{1} \left [ G(k_r + i, k_\theta + j) - H(k_r + i, k_\theta + j) \right ]
    \end{equation}
    Then, a fertile star $s_k$ is selected among the candidates (and marked, so that it will no be used in the following iterations) by means of a biased sampling without replacement, proportional to $f$. In such a way, it is promoted the creation of branches directed towards the most empty cells of the zone.
    \item Now, $m$ new successors states are going to be created by appending up to to each of the $m_0$, already generated, (partial) successor states in $\mathcal{L}$ a different group of offspring of star $s_k$.
    
    
    
    In order to devise an appropriate value for $n_{succ}^k$, a greater ``weight'' has been given to the best stars according to $f$, so that to further encourage exploration:
    \begin{equation}
    \begin{array}{cc}
         n_{succ}^k &=
         \begin{cases}
         1.2\, n_{succ}^{u} & \mbox{if}\,\,\, f_k > \bar{f} \\
         n_{succ}^{u} & \mbox{otherwise}
         \end{cases}
    \end{array}
    \label{eq:nsucck}  
    \end{equation}
    where $n_{succ}^{u} = \left \lfloor b_{f,max}^{\frac{1}{n_{f}}} \right \rfloor$ is the number of successors that each of the $n_{f}$ fertile stars should generate so that to reach a total of $b_{f,max}$, and $\bar{f}$ is the average fitness of the fertile stars.
    \item The number of offspring $n_{o}^k$ of the star $s_k$, to insert in each of the $n_{succ} \times n_{succ}^k$ new successors, is sampled in the range $\left [1, 3 - | \mathcal{O}_k | \right]$ with a probability proportional to itself. 
    The aim is to rapidly increase the number of settled stars in the settlement tree.
    \item Finally, each offspring star $s_o$
    %, reached by the out-bounding Settler Ships,
    must be selected within the neighborhood $\mathcal{N}_k$ of the parent star $s_k$.
    Settler Ship mobility charts suggested that a good strategy to fill, the fastest as possible, all the cells composing a zone is to alternate great ``leaps'' from cell to cell, moving along rows, and quick ``reproduction'' phases, for expanding along columns; such a strategy was named \textit{throw and multiply}:
    \begin{equation}
    \begin{array}{cc}
         s_o &=
         \begin{cases}
         \argmin_{s_h \in \mathcal{N}_k} (t_h - t_k) & \mbox{if}\,\,\, p_r < 0.5 \\%[10pt]
         \argmax_{s_h \in \mathcal{N}_k} \frac{|\Delta \theta_f|}{t_h - t_k} & \mbox{otherwise}
         \end{cases}
    \end{array}
    \label{eq:succ_choice}  
    \end{equation}
    being $p_r$ a random number between 0 and 1 and $\Delta \theta_f$ the difference in final polar angle between star $s_h$ and $s_k$.
    At this point, $s_o$ is removed from $\mathcal{N}_k$ and another offspring star is selected with the same rule, until $n_{o}^k$ offspring are generated.
    The $n_{o}^k$ offspring are appended to one of the $n_{succ} \times n_{succ}^k$ successors, and the process is repeated for each of them.
\end{enumerate}
The steps from 1. to 4. are repeated until a number of successors equal to $b_{f,max}$ is generated.



where $t_f(j)$, $t_0(j)$ are the modified departure and arrival times, that account for the  additional transfer time
$\delta(j)$.

 
%	%t_f(j) = t_f(j) + \delta(j) \\
%	& t_f(j) = \bar t_f(j) + \delta(j) \\
%	& t_0(j) = \bar t_0(j) + \sum_{i=1}^{N}{ M(i,j) \delta(i)} && 


\begin{align}
	\min_{\delta_{min} \le \delta  \le \delta_{max}} & { \sum_{j=1}^{N} { \Delta V(j) }    }
	\\
	\begin{split}
	&  \Delta V =  \overline{ \Delta V} 	+ \tfrac{\partial\Delta V}{\partial t_0} \left(t_0(j) - \bar t_0(j) \right)
	+\tfrac{1}{2} \tfrac{\partial^2\Delta V}{\partial t_0^2} \left(t_0(j) - \bar t_0(j) \right)  \\
	& \phantom{\Delta V =   \Delta V }	 
	+ \tfrac{\partial\Delta V}{\partial t_f} \left(t_f(j) - \bar t_f^(j) \right)
	+\tfrac{1}{2} \tfrac{\partial^2\Delta V}{\partial t_f^2} \left( t_f(j) - \bar t_f^(j) \right)   
	\end{split} \\
	%
	%t_f(j) = t_f(j) + \delta(j) \\
	& t_f(j) = \bar t_f(j) + \delta(j) \\
	& t_0(j) = \bar t_0(j) + \sum_{i=1}^{N}{ M(i,j) \delta(i)} && 
\end{align}

%$a = \dfrac{\partial\Delta V}{\partial t_0}$, 
%$b = \dfrac{\partial^2\Delta V}{\partial t_0^2}$, 
%$c =  \dfrac{\partial\Delta V}{\partial t_f}$, and 
%$d = \dfrac{\partial^2\Delta V}{\partial t_f^2}$



\hl{dice se la stella i is a (non-necessarily immediate) parent of the star $j$
}




\begin{equation}
        \Delta V = \sum_{i=0}^N {\Delta V^i (t_0^i,t_f^i)}     
\end{equation}



where 


%$\Delta V$



The new arrival time $t_f(j)$ is readily obtained.
This modifies all

(22) ha tutta l'aria di essere sbagliata





\hl{tutta da rifare}







